Locally Decodable Codes with Randomized Encoding

We initiate a study of locally decodable codes with randomized encoding. Standard locally decodable codes are error correcting codes with a deterministic encoding function and a randomized decoding function, such that any desired message bit can be recovered with good probability by querying only a small number of positions in the corrupted codeword. This allows one to recover any message bit very efficiently in sub-linear or even logarithmic time. Besides this straightforward application, locally decodable codes have also found many other applications such as private information retrieval, secure multiparty computation, and average-case complexity. However, despite extensive research, the tradeoff between the rate of the code and the number of queries is somewhat disappointing. For example, the best known constructions still need super-polynomially long codeword length even with a logarithmic number of queries, and need a polynomial number of queries to achieve a constant rate. In this paper, we show that by using a randomized encoding, in several models we can achieve significantly better rate-query tradeoff. In addition, our codes work for both the standard Hamming errors, and the more general and harder edit errors.

==> randEncLDC.tex <==
\section{Random Encoding LDC for Hamming Errors}

 
\begin{definition}
		[Locally Decodable Code for Hamming Error]
		
		An ($r$,$\delta$)-locally decodable code is a pair of algorithms $\{\mathbf{Enc},\mathbf{Dec}\}$, such that:
		
		\begin{itemize}
		
			\item $\mathbf{Enc}:\{0,1\}^k\rightarrow \{0,1\}^n$ is the encoding algorithm. For every message $x\in \{0,1\}^k$, $ y = \mathbf{Enc}(x,r) \in \{0,1\}^n$ is a corresponding codeword.
			
			\item $\mathbf{Dec}:[k]\times\{0,1\}^* \rightarrow \{0,1\}$ is the decoding algorithm. For every $i\in [k]$, if $d_E(w,\mathbf{Enc}(x))\leq \delta$, we have
			\[ Pr[\mathbf{Dec}(i,w) = x_i] \geq 2/3 \]
			the probability is taken over $\mathbf{Dec}$'s coin tosses.
			
			\item $\mathbf{Dec}$ makes $r$ queries to $y$.
			
		\end{itemize}
		
	\end{definition}
 
